Fair and Truthful Mechanisms for Dichotomous Valuations

We consider the problem of allocating a set on indivisible items to players with private preferences in an efficient and fair way. We focus on valuations that have dichotomous marginals, in which the added value of any item to a set is either 0 or 1, and aim to design truthful allocation mechanisms (without money) that maximize welfare and are fair. For the case that players have submodular valuations with dichotomous marginals, we design such a deterministic truthful allocation mechanism. The allocation output by our mechanism is Lorenz dominating, and consequently satisfies many desired fairness properties, such as being envy-free up to any item (EFX), and maximizing the Nash Social Welfare (NSW). We then show that our mechanism with random priorities is envy-free ex-ante, while having all the above properties ex-post. Furthermore, we present several impossibility results precluding similar results for the larger class of XOS valuations. To gauge the robustness of our positive results, we also study $\epsilon$-dichotomous valuations, in which the added value of any item to a set is either non-positive, or in the range $[1, 1 + \epsilon]$. We show several impossibility results in this setting, and also a positive result: for players that have additive $\epsilon$-dichotomous valuations with sufficiently small $\epsilon$, we design a randomized truthful mechanism with strong ex-post guarantees. For $\rho = \frac{1}{1 + \epsilon}$, the allocations that it produces generate at least a $\rho$-fraction of the maximum welfare, and enjoy $\rho$-approximations for various fairness properties, such as being envy-free up to one item (EF1), and giving each player at least her maximin share.

==> Definitions.tex <==

There are $n$ agents and $m$ items. Each agent $i$ has a valuation function $v_i$ over sets of items. Each agent $i$ has an entitlement $b_i > 0$ to the items, with $\sum_i b_i = 1$. We seek to allocate the items to the agents in a ``fair" way. We consider first only deterministic allocations, and postpone the treatment of randomized allocations to later (as they require also to model the attitude of agents towards risk).

The interpretation of the entitlement is that every agent $i$ deserves a share of $b_i$ in every item. However, items are indivisible, and hence it is impossible to give each agent his share. An alternative is to try to give the agent items of total value $b_i \sum_j v_i(j)$, but this too might be impossible to do (e.g., when there is just one item).

We present here certain fairness conditions that we may want the allocation to satisfy. They are formulated in terms of the {\em share} of items that the agent receives. The shares are the results that the agent can guarantee to himself in the following games.

\begin{enumerate}

\item {\em Pessimistic share.} The agent may choose arbitrary $p,q > 0$ satisfying $\frac{p}{q} \le b_i$. Thereafter, the agent may partition the items into $q$ bundles of his choice. An adversary then removes $q-p$ of the bundles (in the worst possible way for the agent). The pessimistic share is the value of the set containing the items of the remaining $p$ bundles.

\item {\em Sequential share.} The agent may partition the items into an arbitrary number of bundles. The adversary sets an order among the bundles (worst possible order for the agent). The agent then selects bundles of his choice, with the restriction that from every prefix, the fraction of bundles selected is at most $b_i$.

\item {\em Balanced share.} For $\frac{p}{q} \le b_i$ the agent creates $q$ bundles (that may overlap, or even be identical) such that every item appears in at most (and hence, w.l.o.g, exactly) $p$ of the bundles. The balanced share of the agent is the value of the least valuable of the $q$ bundles.

    Equivalently (one direction of the equivalence is trivial, and the other is not hard), the agent creates an arbitrary number of bundles, associates with them nonnegative weights that sum up to~1, with the following constraint: for every item, the sum of weights that contain it is at most $\frac{p}{q}$. The balanced share of the agent is the value of the least valuable of the positive weight bundles.

    LP duality (to be done) should provide another formulation via prices. The balanced share is the value that an agent with budget equal to his entitlement can guarantee to buy if nonnegative item prices sum to~1.

\end{enumerate}


\begin{example}
Suppose that $b_i = \frac{2}{5}$, that $v_i$ is additive,  and there are six items of values $1,2,3,4,5,6$ (giving total value $21$). The agent may choose $p=2$ and $q=5$, and create the following five bundles: $(1,2)$, $(3)$, $(4)$, $(5)$, $(6)$. With these bundles, the value of the pessimistic share is $6$, but the value of the sequential share is $7$. The agent may also choose $p=1$ and $q=3$ and create the following three bundles: $(1,6)$, $(2,5)$, $(3,4)$.  Here both the values of the pessimistic share and of the sequential share are $7$. For the balanced share, the agent may again choose $p=2$ and $q=5$, but create the following five bundles: $(1,2,5)$, $(1,3,4)$, $(2,6)$, $(3,6)$, $(4,5)$. Every item appears is two bundles, and every bundle is worth at least $8$. Here the balanced share of the agent is $8$. (This is best possible, because $\frac{9}{21} > \frac{2}{5}$).
\end{example}

\begin{proposition}
The sequential share %and the balanced share are each
is at least as large as the pessimistic share. If valuation functions are additive, they are equal whenever the entitlement is $\frac{1}{k}$ for an integer $k$.
\end{proposition}

\begin{proof}
For the sequential share, the agent may form and choose the same bundles as in the pessimistic share.
%For the balanced share, the agent may form $q$ bundles by considering the $q$ bundles that the agent forms for the pessimistic share, taking any $p$ indices of them to form one bundle, and taking the $q$ cyclic shifts of these indices.

When the entitlement is $\frac{1}{k}$, then given the partition for the sequential share sorted in order of decreasing value, one can create $k$ bundles, where bundle $i$ includes those items in parts whose number is $i-1$ mod $k$.
\end{proof}

\begin{proposition}
\label{pro:balancedVersusSequential}
The balanced share is at least as large as the sequential share.
\end{proposition}

\begin{proof}
In the proof we assume w.l.o.g. that for the sequential share, the partition created by the agent is composed of individual items. (If not, each part in the partition can be treated as an item and the proof below still applies.)

Let $\frac{p}{q}$ be the entitlement, and let $c$ denote the value of the sequential share. Let $S_1, S_2, \ldots $ be all those bundles that have value at least $c$, which we shall refer to as feasible bundles. Consider the following LP, associating weight $x_j$ with feasible bundle $j$.

{\em Maximize} $\sum x_j$ {\em Subject to:}

\begin{itemize}

\item $\sum_{j | i \in S_j} x_j \le \frac{p}{q}$ for every item $i$.

\item $x_j \ge 0$ for every feasible bundle $S_j$.

\end{itemize}

It suffices to show that the above LP has value at least~1, as then the balanced share has value at least $c$.

Suppose for the sake of contradiction that the value of the LP is $\rho < 1$, and consider the dual LP, with a variable $y_i$ for every item $i$.

{\em Minimize} $\sum_i \frac{p}{q}y_i$ {\em Subject to:}

\begin{itemize}

\item $\sum_{i | i \in S_j} y_i \ge 1$ for every feasible bundle $S_j$.

\item $y_j \ge 0$ for every item $i$.

\end{itemize}

By strong duality, the value of the dual is also $\rho$. Assign to every item $i$ a price of $p_i = \frac{p}{\rho q}y_i$. Then $\sum p_i = 1$, and for every feasible bundle, the sum of prices of items in the bundle is strictly larger than $\frac{p}{q}$.

For the sequential share, consider an adversarial order from highest value item to lowest value. From every prefix of this order the sequential share can select at most a $\frac{p}{q}$ fraction of the items, and hence the bundle obtained will have price at most $\frac{p}{q}$, contradicting the assumption that the value of the sequential share is $c$.
\end{proof}






\begin{proposition}
\label{pro:CE}
In every competitive equilibrium CE, every agent gets at least his balanced share.
%(for all types of shares listed above).
\end{proposition}

\begin{proof}
In a CE the market clears, and every agent gets the best bundle that he can afford with his budget. As the sum of budgets of agents is~1, the sum of prices of items is at most~1.

%For the pessimistic share, the agent can afford the $p$ cheapest bundles.

%For the sequential share, sort the bundles in order of decreasing prices. For every bundle $s$ picked by the agent, one can charge $s$ against $s$ itself and $\frac{1}{b_i} - 1$ bundles (possibly fractionally) that are priced at least as high as $s$. Hence the agent can afford the bundles that he is allowed to take under the sequential share.

For the balanced share, it cannot be that all bundles are priced above $b_i$ because then the total price of all items is strictly larger than $b_i \frac{p}{q} \ge 1$. Hence the agent can afford at least one of the bundles.
\end{proof}

\subsubsection*{Criteria for reasonableness of fairness concepts}

\begin{enumerate}

\item If all agents have the same entitlement and same valuation, each agent can get at least his share.

\item In a CE each agent gets at least his share.

\end{enumerate}

The pessimistic share and the sequential share satisfy both criteria. We have other notions such as balanced share (that does not satisfy the first criterion) and truncated proportional share (to follow, that does not satisfy any of the criteria). They are useful for proofs, and they offer stronger guarantees when they hold. The notion of WMMS of~\cite{Farhadi+2019} does not satisfy the second criterion. As it also does not dominate the pessimistic share it appears to us not to be a useful notion. (Example, a player with entitlement $\frac{1}{2}$ and items of value 1,1,2,2, where two other players have entitlement of $\frac{1}{4}$ each. The pessimistic share is~3, but WMMS is~2.)

\subsubsection{Additive valuations and the truncated proportional share}

In the special case of additive valuations, we may also consider the {\em proportional share} (which is the total value of the grand bundle times the entitlement). Clearly, agents cannot be guaranteed to receive the proportional share (e.g., if there is only one item). A useful variation is the {\em truncated proportional share}, which is the fixed point of the process of truncating the value of an item so that it does not exceed the proportional share (and recomputing the proportional share, and repeating as long as possible).

\begin{proposition}
The truncated proportional share is at least as large as the balanced share.
\end{proposition}

\begin{proof}
Truncate the value of each item so that it does not exceed the balanced share.
\end{proof}


\begin{proposition}
\label{pro:notTruncated}
There are instances with $n$ agents in which in every allocation, at least one of the agents does not get more than a $\frac{n}{2n-1}$ fraction of his truncated proportional share.
\end{proposition}

\begin{proof}
An instance with $2n-1$ equal valued items.
\end{proof}

\begin{proposition}
In a CE an agent need not get his truncated proportional share.
\end{proposition}

\begin{proof}
Two agents, one agent with entitlement $0.4$ and value $0.36$ for item $A$ and $0.32$ for each of items $B$ and $C$, the other with equal values to the items. Pricing $A$ at $0.4$ and $B$ and $C$ at $0.3$ is a CE.
\end{proof}

\subsection{Negative examples}

A useful class of (monotone) valuation functions is the {\em distinguished sets} class. There is a set $U$ of  $m$ items and a parameter $t$, and a collection of subsets of $U$, each of size $t$, that are referred to as {\em distinguished}. The value of every distinguished set is $t$, and so is the value of any set that contains a distinguished set, including $U$. The value of the empty set is~0. As to the values of other sets, there are four classes:

\begin{enumerate}

\item {\em Submodular:} every set $S$ of size $|S| < t$ has value $|S|$. Sets $S$ of size $|S| \ge t$ that do not contain a distinguished set have value $t - 2^{t -1 - |S|}$.

\item {\em XOS:} the value of a set is the maximum intersection size that it has with a distinguished set.

\item {\em Subadditive:} (nonempty) sets not containing a distinguished set have value $\frac{t}{2}$.

\item {\em General:} sets not containing a distinguished set have value~0.

\end{enumerate}

In propositions that present negative examples we shall typically consider valuations with distinguished sets. The share of every agent will be $t$, but no allocation will be able to give all agents value $t$. We shall typically state the conclusions for the case that valuations are submodular, but stronger conclusions can be drawn for the three other classes. In our negative examples, entitlements sum up to less than~1, and so they also serve as examples in which no competitive equilibrium from generic budgets exists. (See~\cite{BNT17,Segal18} for an explanation of this notion and for other examples.)
%Most propositions were written before introducing the terminology of distinguished sets, but later versions of the manuscript can switch to this terminology and make the examples less repetitive.


\begin{proposition}
\label{pro:entitlementNo}
For every $0 < \rho \le 1$, there are instances with submodular valuation functions in which all agents have the same entitlement $\frac{\rho}{n}$ and no allocation gives every agent his pessimistic share.
\end{proposition}

\begin{proof}
Consider an instance with $k^2$ items arranged in a $k$ by $k$ matrix, and two agents: $R$ (for row) and $C$ (for column).  For the row player the distinguished sets are the rows, and for the column player the distinguished sets are the columns.   No allocation gives both agents value of $k$. However, even with entitlement $\frac{1}{k}$, the pessimistic share of each agent is $k$. Hence choosing $k$ such that $\frac{2}{k} \le \rho$ the proposition follows.
\end{proof}

\begin{proposition}
There are instances with seven items and two agents with identical submodular valuation functions and entitlements $\frac{3}{7}$ (hence summing to less than 1) for which in every allocation an agent does not get his balanced share.
\end{proposition}

\begin{proof}
The distinguished sets are lines in the 7-point projective plane. Every line has 3 points and every two lines intersect. For the balanced share, take all 7 lines, giving each agent a share of 3.
\end{proof}

\begin{proposition}
\label{pro:noBalancedShare}
For every $\frac{1}{2} < \rho \le 1$ there are instances in which all $n$ agents have the same entitlement $\frac{\rho}{n}$ and the same submodular valuation function, and no allocation gives every agent his balanced share. For some $\rho < 1$, the same also holds for sequential share.
\end{proposition}

\begin{proof}
For sufficiently large $k$ satisfying $\frac{k+1}{2k-1} \le \rho$, there are $k(2k-1)$ items and $k+1$ agents, each with entitlement $\frac{\rho}{k+1} \ge \frac{1}{2k-1}$. The items are arranged in $k$ groups, each with $2k-1$ items. The valuation function $v$ of all agents is the same, and its distinguished sets are those sets of size $k$ in which all items are from the same group.
%For every set $S$ of items, if $|S| < k$ then $v(S) = |S|$, if $S$ contains at least $k$ items from some group then $v(S) = k$, and in all remaining cases $v(S) = k - 2^{k - |S| - 1}$. It is not difficult to check that this valuation function is submodular.

In every allocation, at most $k$ agents get value $k$ and the remaining agent gets value strictly smaller than $k$.
%(If we do not care about submodularity, we can choose $v(S) = 1$ if $S$ contains at least $k$ items from some group, and $v(S) = 0$ otherwise, making the remaining agent get value~0.)

With entitlement of $\frac{1}{2k-1}$, the balanced share of every agent is $k$. (Each group can be covered $k$ times by taking $2k-1$ cyclic shifts of a bundle of size $k$.)


If $\rho = \frac{5}{6}$ and $k$ is sufficiently large, then the sequential share is also $k$.  Here is a sketch of proof, omitting terms that tend to~0 as $k$ grows. Consider a partition of the items into $k(2k-1)$ bundles, in which every item is a bundle. Given an adversarial order on these bundles (equivalently, on the items), for an agent with entitlement $\frac{\rho}{n} = \frac{\rho}{k+1} \simeq \frac{\rho}{k}$, the $j$th item that the agent selects can be anywhere starting from location $j\frac{k}{\rho}$, for $1 \le j \le k$. To be able to select $k$ items from the same group, it suffices that there is some group such that for every $1 \le j \le k$, there are at least $k-j+1$ items from the group in the suffix that starts at location $j\frac{k}{\rho}$. Consequently, for the agent not to get $k$ items from the same group, for every group there must be an index $1 \le j \le k$ such that at least $2k-1 - (k - j + 1) + 1 = k + j - 1$ items from the group appear before location $j\frac{k}{\rho}$. Partition the groups into classes according to the $j$ that apply to them. The number of groups in classes up to $j$ is at most $2j$. (Stronger upper bounds apply, and they lead to lower values of $\rho$. Details omitted.) This implies that at least $(k + (k + \frac{k}{2} - 1))\frac{k}{2} \simeq \frac{5}{4}k^2$ items have to appear up to location $\frac{k^2}{\rho}$. But this cannot happen if $\rho = \frac{5}{6}$.

The choice of $\rho = \frac{5}{6}$ is not optimal and is done so as to simplify the proof. The best value of $\rho$ implied by the  example (with sufficiently large $k$) is somewhere between $\frac{1}{2}$ and $\frac{4}{5}$, but we have not attempted to compute it.
\end{proof}


\begin{proposition}
\label{pro:noBalancedShare1}
There are examples in which all agents have identical additive valuation functions and the same entitlement $\frac{1}{n}$, and there is no allocation that gives every agent his balanced share.
\end{proposition}

\begin{proof}
We design an example with 15 items and three agents. The items will be named $x_{ij}$ for $1 \le i < j \le 6$. To simplify notation, we will also allow the usage of $x_{ii}$ even though there is no such item (one may think of $x_{ii} = 0$), and of $x_{ji}$ with $1 \le i < j \le 6$, which will serve as an alternative name for $x_{ij}$.

The values that we give to the items in the proof are taken from a large range of values. This is done so as to simplify the presentation. One can significantly narrow this range with extra work.

Let $M$ be a sufficiently large even constant, such as $M = 2^{20}$. The ten items $x_{ij}$ for $1 \le i < j \le 5$ have the ten values $M + 2^k$ for $1 \le k \le 10$ (at an arbitrary order). Observe that all values are roughly $M$, and even. Let $S = \sum_{1 \le i < j \le 5} x_{ij}$, and observe that $\frac{S}{2}$ is odd.

For the remaining five items $x_{i6}$ for $1 \le i \le 5$, their value is $x_{i6} = \frac{S}{2} - \sum_{1 \le j \le 5} x_{ij}$. Observe that the value of $x_{i6}$ is roughly $M$ and odd.

The total value of all items is $S + \sum_{1 \le i \le 5} x_{i6} = S + 5\frac{S}{2} - 2S = \frac{3S}{2}$.

The balanced share (of every agent, as they have identical valuations) is $\frac{S}{2}$. This can be seen by creating six bundles, where every item appears in two of the bundles. For every $1 \le i \le 6$ there is a bundle that contains the five items $x_{ij}$ for $j \not= i$. For the first five bundles their value is $x_{i6} + \sum_{1 \le j \le 5} x_{ij} = \frac{S}{2}$. The value of the last bundle is $\sum_{j\not= 6} x_{6j} = \sum_{i\not= 6} x_{i6} = 5\frac{S}{2} - 2S = \frac{S}{2}$.

We now show that in every allocation at least one of the agents gets a bundle of value smaller than $\frac{S}{2}$. Suppose otherwise. Then every agent gets value exactly $\frac{S}{2}$ (because the total value is $\frac{3S}{2}$). As  $\frac{S}{2}$ is odd, every agent needs to get an odd number of items from the set $\{x_{i6}\}_{1 \le i \le 5}$. Hence two agents need to each get exactly one item from this set. W.l.o.g., one of them gets $x_{16}$ and the other $x_{26}$. In addition, each of them needs to get exactly four other items (so that his value would be roughly $5M \simeq \frac{S}{2}$). But the only four items that make the first bundle have value $\frac{S}{2}$ are $\{x_{1j}\}_{2 \le j \le 5}$, and the only four items that make the second bundle have value $\frac{S}{2}$ are $\{x_{2j}\}_{j \in \{1,3,4,5\}}$. Hence item $x_{12} = x_{21}$ is allocated twice, whereas it can be allocated only once.
\end{proof}

The following theorem was proved in~\cite{KPW18}.

\begin{theorem}\cite{KPW18}
For every $n \ge 3$, there are instances with $n$ agents, additive valuation functions and equal entitlements, in which there is no allocation that gives every agent his pessimistic share.
\end{theorem}


\begin{example} [Example why there is no truthful proportional mechanism] \te{move to truthful}
	Consider the case of two agents with 3 items and entitlements $b_1=0.65, b_2=0.35$.
	$v_1(1)=80,v_1(2)=10, v_1(3)=10$,
	$v_2(1)=40,v_2(2)=35, v_2(3)=25$.
	There are two proportional allocations (agent 1 gets 1,3, and agent 1 gets only 1)
	If agent 1 reports 	$v_1(1)=40,v_1(2)=30, v_1(3)=30$, he can guarantee that he gets $1,3$. If agent 2 reports 	$v_2(1)=40,v_2(2)=30, v_2(3)=30$ he can guarantee that he gets $2,3$.	
\end{example}
\begin{example}	[Example why there is no truthful pessimistic mechanism] \te{move to truthful}
	Consider the case of two agents with 4 items and entitlements $b_1=0.5, b_2=0.5$.
	$v_1(1)=7,v_1(2)=1, v_1(3)=1,v_1(4)=1$,
	$v_2(1)=7,v_2(2)=1, v_2(3)=1, v_2(4)=1$.
	W.L.O.G agent 2 gets items 2,3,4.
	if agent 2 reports
	$v_2(1)=1,v_2(2)=4, v_2(3)=2, v_2(4)=3$.
	\te{fix}
	
	There are two allocations that give each agent its pessimistic share (agent 1 gets 1,2, and agent 1 gets only 1)
	If agent 1 reports 	$v_1(1)=40,v_1(2)=30, v_1(3)=30$, he can guarantee that he gets $1,3$. If agent 2 reports 	$v_2(1)=40,v_2(2)=30, v_2(3)=30$ he can guarantee that he gets $2,3$.
\end{example}

\begin{example}[cannot partition the items such that all players have a value half of $b$]
	Consider a market with 2 agents and 3 items:
	$v_1(1)=1/4,v_1(2)=3/8, v_1(3)=3/8$,
	$v_2(1)=1/2,v_2(2)=1/4, v_2(3)=1/4$.
	In every partition there exists an agent with value $1/4$ for one of the bundles.
\end{example}

\begin{example}[Example why the items value must be bounded by $\frac{2b}{3}$]
	Consider a market with n=2k-1 agents and 3k-2 items:
	agent $i$ has a value of $\frac{1}{3k-3}$ for every item except for item $i$.
	In every partition into $n$ non-empty bundles there exists one of the first $n$ items alone in a bundle. This bundle has a value of $0$ for agent $i$.
	In order to Guarantee value for each agent to each bundle we need an assumption like $v_i(j) \leq \frac{2}{3n}$.
\end{example}




\subsection{Positive results}

\begin{proposition}
\label{pro:equalYes}
If all agents have the same entitlement and the same valuation function, then there is an allocation that gives each agent his pessimistic share. If moreover the valuation function is additive, then there is an allocation that gives each agent his sequential share.
\end{proposition}

\begin{proof}
Consider the partitioning into $q$ bundles with $\frac{p}{q} \le \frac{1}{n}$ that determines the pessimistic share of an agent (and hence of every agent). Giving each agent a different set of $p$ bundles from this partition guarantees that each agent receives at least his pessimistic share.

Consider a partition into bundles for the sequential share, and let $\frac{p}{q} \le \frac{1}{n}$ be the maximal ratio of bundles taken by the agent from any prefix of the adversarial order. If needed, add empty bundles to the suffix of the order so that the number of bundles $k$ is divisible by $q$, and add to the agent additional bundles so that his total number of bundles is $\frac{p}{q}k$, not taking more than a fraction of $\frac{p}{q}$ bundles from any prefix.

Beyond the collection of bundles that the agent receives in his sequential share, we can create $n-1$ additional collections by shifts of the selected bundles, where all shifts are only made upwards. (The proof that this process does not get stuck is not difficult, but omitted.)
\end{proof}

\begin{proposition}
\label{pro:unitDemand}
If all valuation functions are unit demand, then there is an allocation giving each agent at least his balanced share.
\end{proposition}

\begin{proof}
The balanced share of a unit demand agent with entitlement $0 \le b \le 1$ is his $\lceil \frac{1}{b} \rceil$ most valued item. Sort agents in order of decreasing entitlement (breaking ties arbitrarily) and let them each choose an item at his turn. As entitlements sum up to~1, the turn of an agent with entitlement $0 \le b \le 1$ comes no later than step $\lceil \frac{1}{b} \rceil$, and hence he may choose an item of value at least his balanced share.
\end{proof}

We introduce of the following {\em allocation game}. The agents are the players in the game. The game proceeds in rounds, where the number of items is the number of rounds. Initially, each player gets a budget equal to his entitlement. Thereafter, in each round, an auction is held. Every player may place a bid in this auction, of value not larger than his remaining budget. The highest bidder wins (breaking ties arbitrarily), and pays his bid. (The theoretical results that we present stay the same if instead the winner pays the second highest bid. The second price auction version may be preferable if one would like to implement this auction in practice.) Thereafter the winner chooses an item of his choice and the round ends.

Given the valuation function of an agent, his entitlement, and the entitlements of the other agents, the maxmin value for the player in the game is the maximum sum of value of received items that the agents can guarantee to himself no matter how the other agents play. As this maxmin value is guaranteed by some deterministic strategy for the player, it follows that there is a single allocation that gives every player his maxmin game value.

We shall also consider a stand alone maxmin value, which assumes that all other players are replaced by a single player whose budget equals the sum of their budgets. This value can be computed by an agent without knowing the entitlements of other agents (because the sum of all entitlements are~1), and is never larger than the game maxmin value.

We always assume that additive valuation functions are normalized so that the grand bundle has value~1, and that the sum of entitlements is~1.

\begin{theorem}
\label{thm:safeStrategy}
For an agent with additive valuation function and entitlement $b$, if for some positive integer $t$ no item has value more than $b/t$, then the stand alone share of the agent is at least $(1 - \frac{1}{t+1})b$.
\end{theorem}

\begin{proof}
Consider first the case that $t = 1$. Then we propose the following strategy for the agent. Let the budget avialble to the agent at the begining of round $i$ be $b_i$ (with $b_1 = b$). If there is an item of value at least $\frac{b_i}{2}$, bid $b_i$. Otherwise, bid the value of the most valuable item. If a round is won, select the highest value item among the remaining ones. This strategy maintains the property that as long as the agent has budget left, the rate at which his budget is consumed is is the same as the rate at which he accumulates value, whereas the rate at which budget of other is consumed is at least as large as the rate at which the value of the remaining items decrease. If this property is maintained throughout the game, then necessarily the agent gets a value of at least $b$. There are only two ways in which this property might fail to hold:

\begin{enumerate}

\item At a round $i$ there is an item of value larger than $b_i$. This can happen (for the first time) only if the player won round $i-1$. But then he selected an item of value larger than $b_i$, and so his total value is already above $b/2$.

\item At round $i$ the agent bid $b_i$ but won an item of smaller value. But then the value of this item is at least $b_i/2$, and the total value of his items reaches at least $b/2$.

\end{enumerate}

Now we prove the theorem for general $t > 1$ by induction. The agent follows exactly the same strategy as above. Let $i$ be the first round in which there is  an item of value $v_i > b_i/2$. Necessarily, $b_i < \frac{2b}{t}$. Up to round $i$ the property referred to above holds, and the agent accumulated a value of $b - b_i$. It cannot be that $v_i > b_i$ as then already in round $i-1$ the agent got an item worth more than half his budget for the round, contradicting the minimality of $i$.
Hence $v_i \le b_i$, and if $b_i \le \frac{2}{t+1}b$, then the theorem follows from the case $t=1$. Hence every item won by the agent up to round $i$ had value between $\frac{b_i}{2} > \frac{b}{t+1}$ and $\frac{b}{t}$. But this cannot happen if the budget left for the agent satisfies $\frac{b}{t+1} < b_i < \frac{2b}{t}$.
\end{proof}

The following theorem should be true.

\begin{theorem}
\label{thm:safeStrategy1}
For an agent with additive valuation function and entitlement $b$, if no item has value above $b$, the stand alone share of the agent is at least $\frac{b}{2-b}$.
\end{theorem}

\begin{proof}
(Sketch -- perhaps needs change.) We propose the following strategy. In every round,  do the following:

\begin{itemize}

\item Rescale all budgets so that they sum up to~1, and rescale the value of all items so that they sum up to~1. If as a result, there are items of value above the current budget $b$, find the largest threshold $t$ such that changing the value $v(i)$ of each item $i$ to $\min[v(i),t]$ and rescaling so that values sum up to~1 corrects this situation. If no such $t$ exists, abort. Thereafter:
\te{isn't the capping redundant since in the theorem we assume that $v\leq b$}

\item If there is an item of value at least $\frac{b}{2-b}$, then bid $b$.

\item Else, if there is an item of value above $\frac{1}{2}$, bid $\frac{1}{2}$.

\item Else bid the value of the most valuable item.

\end{itemize}
The proof can (hopefully) be by induction on the number of items left.
\end{proof}


For $m$ items, entitlement $b$ out of $B$ and values $v=(v_1,\ldots,v_m)$ such that $v_1 \geq \ldots \geq v_m$ and $\sum_i v_i=s_v$, and $\frac{v_1}{s_v} \leq \frac{b}{B}$,

Agent's strategy:
\begin{itemize}
	\item if $v_1 \geq \frac{s_v \cdot b}{2B-b}$ bid $b$
	\item if $\frac{s_v \cdot b}{2B-b}>v_1 \geq \frac{s_v b}{2B}$ bid $\frac{b}{2}$
	\item else bid $\frac{v_1\cdot B}{s_v} (\leq \frac{b}{2})$
\end{itemize}

\begin{theorem}
	we prove that the agent's value when using this strategy is at least $\frac{s_v \cdot b}{2B-b}$. (not normalized version of Theorem \ref{thm:safeStrategy1}) \te{finish this proof}
\end{theorem}

\begin{proof}
	

Proof of correctness:
We prove by induction over the number of remaining items.
If the number of items is $1$, then it must be that $v=(1)$ and $b=B$ (by the assumption that $\frac{b}{B} \geq \frac{v_1}{s_v}=1$), therefore the agent will be the only contestant and will win the item.
We assume for $m$ items.
For $m+1$ items, we divide into case:
%we prove that for an entitlement $b$ out of $B$ and valuation $v=(v_1,\ldots,v_m,v_{m+1})$ such that $b\geq v_1 \geq \ldots \geq v_{m+1}$,  and $\sum_i v_i=s_v$, and $\frac{v_1}{s_v} \leq \frac{b}{B}$, the agent's maxmin value is at least $\frac{s_v \frac{b}{B}}{2-\frac{b}{B}}$.

\begin{itemize}
	\item $v_1 \geq \frac{s_v \cdot b}{2B-b}$ and the agent won the item - trivial.
	\item $v_1 \geq \frac{s_v \cdot b}{2B-b}$ and another agent won the item (and paid $b$), then by the assumption holds since $\frac{v_1^{new} }{s_v^{new}} \leq \frac{v_1}{s_v-v_1} \leq \frac{b}{B-b} =  \frac{b^{new}}{B^{new}},$ where the second inequality follows by the assumption.
	Therefore by induction the value is at least $\frac{s_v^{new} \cdot b^{new}}{2B^{new}-b^{new}} \geq \frac{(s_v -v_1) \cdot b}{2(B-b)-b} \geq \frac{(s_v -s_v\frac{b}{B}) \cdot b}{2(B-b)-b} \geq \frac{s_v \cdot b}{2B-b}.$
	\item $\frac{s_v \cdot b}{2B-b}>v_1 \geq \frac{s_v b}{2B}$ and the agent won the item.
	As long as
	$\frac{b^{new}}{B^{new}} < \frac{v_1^{new}}{s_v^{new}}$, the agent bids $b^{new}=b/2$. if the agent wins an item during this phase (assume that he wins an $k$-th item), his value
	$v_1^{new}>\frac{s_v^{new} \cdot b^{new}}{2B^{new}-b^{new}}=\frac{(s_v-v_1)}{}$,
	
	
	
	
	the induction assumption holds since:
	$\frac{v_1^{new} }{s_v^{new}} = \frac{v_2}{s_v-v_1} \leq \frac{b/2}{B-b/2} =  \frac{b^{new}}{B^{new}},$
	\te{this case is not a direct induction since the values can exceed the budget, but item still need to be paid at least $b/2$ until the assumption will hold again, if another item will be bought during this process then we are done.}
	
	\te{need to prove for the case where $\frac{b}{B}>\frac{1}{2}$ with that can look at what remains after selling $k=\lfloor \frac{1-b/2}{b/2}\rfloor$ items.}
	\item $\frac{s_v \cdot b}{2B-b}>v_1 \geq \frac{s_v b}{2B}$, and another agent won the item for a price of $\frac{b}{2}$.
	The induction assumption holds since
	$\frac{v_1^{new} }{s_v^{new}} \leq min(1,\frac{v_1}{s_v-v_1}) \leq min(1,\frac{\frac{s_v \cdot b}{2B-b}}{s_v-\frac{s_v \cdot b}{2B-b}}) = min(1,\frac{b}{2B-2b})  \leq \frac{b}{B-b/2} =  \frac{b^{new}}{B^{new}}.$
	Therefore by induction the agents value is at least $\frac{s_v^{new} \cdot b^{new}}{2B^{new}-b^{new}} \geq \frac{(s_v -v_1) \cdot b}{2(B-b/2)-b} \geq \frac{(s_v -\frac{s_v \cdot b}{2B-b}) \cdot b}{2(B-b)-b} =\frac{b\cdot s_v \cdot (2B-2b)}{(2B-3b)(2B-b)}  \geq \frac{s_v \cdot b}{2B-b}.$
	\item $v_1< \frac{s_v b}{2B}$, and the agent won the item (and paid $\frac{v_1\cdot B}{s_v}$).
	The induction assumption holds since
	$\frac{v_1^{new} }{s_v^{new}} \leq \frac{v_1}{s_v-v_1}  \leq  \frac{\frac{s_v b}{2B}}{s_v-v_1}
	= \frac{b/2}{B-\frac{v_1\cdot B}{s_v}} \leq \frac{b-\frac{v_1\cdot B}{s_v}}{B-\frac{v_1\cdot B}{s_v}} =  \frac{b^{new}}{B^{new}}.$
	Therefore the agent value by the induction is at least $v_1 + \frac{s_v^{new} \cdot b^{new}}{2B^{new}-b^{new}} =v_1 + \frac{(s_v-v_1) \cdot (b-\frac{v_1\cdot B}{s_v})}{2(B-\frac{v_1\cdot B}{s_v})-(b-\frac{v_1\cdot B}{s_v})} = v_1 + \frac{(s_v-v_1) \cdot (s_v\cdot b-v_1\cdot B)}{2s_v \cdot B-v_1\cdot B-s_v\cdot b}=  \frac{2v_1\cdot s_v \cdot B - v_1^2\cdot B-v_1 \cdot s_v \cdot b + s_v^2\cdot b-s_v\cdot v_1\cdot B  -v_1\cdot s_v\cdot b +v_1^2\cdot B}{2s_v \cdot B-v_1\cdot B-s_v\cdot b} =  \frac{v_1\cdot s_v \cdot B -2v_1 \cdot s_v \cdot b + s_v^2\cdot b}{2s_v \cdot B-v_1\cdot B-s_v\cdot b}
	\geq \frac{s_v \cdot b}{2B-b}$
	\item $v_1< \frac{s_v b}{2B}$, and another agent won the item (and paid $\frac{v_1\cdot B}{s_v}$).
	The induction assumption holds since
	$\frac{v_1^{new} }{s_v^{new}} \leq \frac{v_1}{s_v-v_1}  \leq  \frac{\frac{s_v b}{2B}}{s_v-v_1}
	= \frac{b/2}{B-\frac{v_1\cdot B}{s_v}} \leq \frac{b}{B-\frac{v_1\cdot B}{s_v}} =  \frac{b^{new}}{B^{new}}.$
	Therefore the agent value by the induction is at least $\frac{s_v^{new} \cdot b^{new}}{2B^{new}-b^{new}} \geq
	\frac{(s_v -v_1)b}{2(B-\frac{v_1\cdot B}{s_v})-b}
	 \geq \frac{s_v \cdot b}{2B-b}$
		
	
\end{itemize}

\end{proof}


\begin{remark} It would be interesting to see what gaurantee one gets by running the strategy of Theorem~\ref{thm:safeStrategy1} when there is no item of value larger than $\frac{b}{t}$ (for integer $t$, or perhaps even non-integer).
\end{remark}

\begin{theorem}
\label{thm:2/k}
Suppose that for integer $k \ge 3$ and an agent of budget $b = \frac{2}{k}$, one can partition the items into $k$ bundles such that the value of each bundle is at least~1. Then the stand alone share of the agent is at least $\frac{3}{2}$.
\end{theorem}

\begin{proof}
(Sketch.) As long as possible, bid the value of the highest valued item. (We assume that if the adversary wins the bid he pays our bid and takes our most desirable item.) When no longer possible, the budget left must be between $\frac{1}{2}$ (otherwise we are done) and  $\frac{2}{3}$. Bid all budget on any item of value more than $\frac{1}{2}$. At worse, the adversary wins all such items $\frac{2}{3}$ and pays at least $\frac{1}{2}$ for each. Up to this point, at most $k$ items are consumed, and no item left has value above $\frac{1}{2}$. We continue to bid all our budget on any sufficiently valuable item (that makes our total value reach $\frac{3}{2}$, and afterwards only small items remain, and finishing should be easy.
\end{proof}
%'
\begin{corollary}
\label{cor:safeStrategy}
There is an allocation giving every agent at least $\frac{3}{5}$ fraction of his pessimistic share.
\end{corollary}

\begin{proof}
(Sketch.) Lets first prove $\frac{4}{7}$. As long as there is an item of value at least $\frac{4b}{7}$, bid $b$. Thereafter, truncate the value of each item at $\frac{3b}{7}$, rescale the valuation function so that it sums to~1, and apply Theorem~\ref{thm:safeStrategy} with $t=2$.

To get $\frac{3}{5}$,  as long as there is an item of value at least $\frac{3b}{5}$, bid $b$. Thereafter, truncate the value of each item at $\frac{2b}{5}$, rescale the valuation function so that it sums to~1, and apply Theorem~\ref{thm:2/k}.
\end{proof}


\begin{proposition}
\label{pro:Neg2/3}
There are instances with $k$ agents and equal entitlements in which the maxmin value of the allocation game is at most $\frac{2}{3} + O(\frac{1}{\sqrt{k}})$ of the pessimistic share.
\end{proposition}


\begin{proof}
There are $k$ bundles. In $k-1$ bundles there is one heavy item of value~$\frac{2}{3}$ and one medium item of value~$\frac{1}{3}$. In the remaining bundle there are $k$ light items of value $\frac{1}{k}$.  The pessimistic share is one bundle and gives value~1.

The adversary places bids of $\frac{1}{2} + \frac{1}{\sqrt{k}}$ in the first $\frac{k-1}{2}$ rounds. If the agent wins any of these rounds, then the adversary places bids of $\frac{1}{2} - \frac{1}{\sqrt{k}}$ on all the remaining heavy and medium items, winning them, and still has $\Omega(\sqrt{k})$ budget for the light items.

If the adversary wins the first $\frac{k-1}{2}$ rounds, then he places bids of $\frac{1}{2} + \frac{2}{\sqrt{k}}$ on the next $\frac{k-1}{2}$ rounds. If the agent wins one of these rounds, then the adversary places bids of $\frac{1}{2} - \frac{2}{\sqrt{k}}$ on all the medium items, winning them, and still has $\Omega(\sqrt{k})$ budget for the light items.

If the adversary wins all heavy items, he places bids of $\frac{1}{2} - \frac{2}{\sqrt{k}}$ on all the medium items, so he still has a budget of $\Omega(\sqrt{k})$ for the light items. The agent can win at most two medium items.

In any case, the agent wins at most an $O(\frac{1}{\sqrt{k}})$ of the light items.
\end{proof}

The strategy of the adversary in Proposition~\ref{pro:Neg2/3} is not monotone -- his bids increase with time. It would be interesting to see if restricting strategies in the allocation game to be monotone improves the maxmin value. (Probably not, as this also restricts the agent.)

A natural variation on the allocation game (natural if one is interested in improved approximation of the pessimistic share) is to have a parameter $0 \le \alpha \le 1$, and alow agents to bid only if the budget that they have (before the bid) is at least a $\alpha$-fraction of their original budget. For $\alpha > \frac{1}{\sqrt{k}}$ the adversarial strategy in Proposition~\ref{pro:Neg2/3} is not legal in the $\alpha$-game. Here is an example of a negative result in the $\alpha$-game.

\begin{proposition}
\label{pro:Neg2/3}
For $\alpha = \frac{1}{4}$ there are instances with $k$ agents and equal entitlements in which the maxmin value of the $\alpha$-allocation game is at most $\frac{6}{7} + O(\frac{1}{k})$ of the pessimistic share.
\end{proposition}

\begin{proof}
There are $k$ bundles, each with one heavy item of value~$\frac{4}{7}$ and $k$ light items of value $\frac{3}{7k}$.  The pessimistic share is one bundle and gives value~1.

For the first $k$ rounds, if the agent ever bids above $\frac{1}{2}$ the adversary lets him win, and wins the remaining with bids of $\frac{1}{2}$. This exhausts the budget of $\frac{k-1}{2}$ of the adversarial agents. Hence $\frac{k-1}{2}$ adversarial agents remain with their full budget, and our agent has only half its budget. As only light items remain and agents need to stop bidding when their budget reaches $\alpha = \frac{1}{4}$, then effectively the budget of our agent is $\frac{1}{4}$ and that of the adversary is $\frac{3k}{8}$ (up to low order terms). Hence the agent can win a fraction of $\frac{2}{3k}$ of the remaining items, giving him additional value of $\frac{2}{7}$.

If the agent does not bid above $\frac{1}{2}$ in the first $k$ rounds, the adversary wins all heave items, and still has $\frac{k-1}{2} - 1$ adversarial agents left. Hence our agent wins roughly a $\frac{2}{k}$ fraction of the light items, giving total value of $\frac{6}{7}$.
\end{proof}

One can be optimistic that for an appropriate choice of $\alpha$ one can use the $\alpha$-game to get an approximation of the pessimistic share that it better than that given when $\alpha = 0$. Here is a strategy that maybe achieves $\frac{3}{4}$ when $\alpha=\frac{1}{4}$ and there are $k$ agents of equal entitlement. In every round, use the first rule applicable.

\begin{enumerate}

\item If there is an item such that winning it completes the value to at least $\frac{3}{4}$, bid all your budget.



\item For integer $t \ge 2$, if there are $t$ items such that winning them completes the value to at least $\frac{3}{4}$, and the budget is more than $t$ times higher than that of every adversarial agent, then bid a $1/t$ fraction of the budget on each of these items.


\item If there is an item of value $\frac{1}{2} < v < \frac{3}{4}$ bid $\frac{v}{2} + \frac{1}{4}$.

\item Bid the value of the highest valued item.

\end{enumerate}

Steps~1, 2 and~4 above are natural. Step~3 is added so as to give the bidder a buffer from $\alpha$ after winning his first item. Without Step~2 there is the following counter example: $\frac{k-1}{2}$ bundles with $(\frac{3}{4}, \frac{1}{4})$, $\frac{k-1}{2}$ bundles with $(\frac{5}{8}, \frac{3}{8}^-, 0^+)$, and one bundle with  $(\frac{7}{16}, \frac{7}{16}, \frac{1}{8})$. With Step~3 the last bundle needs to be changed to $(\frac{3}{8}^-, \frac{3}{8}^-, \frac{1}{4}^+)$.



The following results have been proved in~\cite{KPW18,AMNS17,Ghodsi+2018}.

\begin{theorem}
With equal entitlements, there are allocations that approximate the pessimistic share within the following ratios for the respective valuation classes:
\begin{itemize}
\item Additive: $\frac{3}{4}$ (and $\frac{7}{8}$ for $n=3$ and $\frac{4}{5}$ for $n=4$).
\item Submodular: $\frac{1}{3}$ (and $\frac{3}{4}$ is an upper bound).
\item XOS: $\frac{1}{5}$ (and $\frac{1}{2}$ is an upper bound).
\item Subadditive: $\frac{1}{10\log m}$.
\end{itemize}
\end{theorem}

\begin{theorem}
	Any truthful mechanism for 2 players, when bidders valuation for each item is bounded by $c$ cannot give better approximation ratio than $O(mc)$.
\end{theorem}
\begin{proof}
	In \cite{??} they characterize all the truthful mechanisms, and show that a truthful mechanism can be described as a partition of the items into 4 sets $A_1,A_2,B_1,B2$ and a set of potential swaps between $A_1$ and $A_2$, and two collections of set $C_1,C_2$ where $C_i \subseteq P(B_i)$, and each agent $i$ chooses one of the sets in $C_i$ where the other agent gets its compliment.
	
	Assume w.l.o.g. that $|A_1|+|B_1| \geq \frac{m}{2}$
	Let $X$ be the largest set in $C_1$. If $|A_1|+|X| \geq \frac{1}{c}$, then consider the valuation of both players to be such that all of the value is spread equally among  $A_1 \cup X$. It is easy to verify that in this case the value of agent 2 will be 0.
	If $|A_1|+|X| < \frac{1}{c}$, consider the valuation for both players to be such that all of the value is spread equally among  $A_1 \cup B_1$. It is easy to verify that in this case the value of agent 1 will be $\frac{|A_1 \cup X|}{|A_1 \cup B_1|} \leq \frac{1/c}{m/2}=\frac{2}{mc}$.
\end{proof}



\subsection{Properties of fairness}
******************generalize definition to any number of agents on order for the union property to be well defined.*********************


An allocation rule $f$ is a function that gets valuation functions $v=(v_1,\ldots,v_n)$ and entitlements $b=(b_1,\ldots,b_n)\neq \bar{0}$ and returns a fair allocation (or a set of fair allocations).
There are some natural properties that we may want this function to have:
\begin{itemize}
	\item \textbf{monotonicity}: $b_i' \geq b_i \implies
	v_i(f(v,b_1,\ldots b_i',\ldots, b_n)_i) \geq v_i(f(v,b_1,\ldots b_i,\ldots, b_n)_i).$
	\item \textbf{scaling}: for $b,v$ and $\alpha>0, $ $f(v,b) =
	f(v,\alpha\cdot  b).$
	\item \textbf{anonymity}:
	for all $i,j,v,b$: $$f_j(swap_{i,j}(v),swap_{i,j}(b)) = f_i(v,b),$$
	where $swap_i,j(v)$ is the vector where the $i$-th and $j$-th entries are swapped.
	\item  \textbf{union}: if $v_i=v_j$ then $f_i(v,b) + f_j(v,b) \leq f_1(v_i,v_{-i,j},b_i+b_j,b_{-i,j}),$
	\item \textbf{proportional}:
	If there exists a proportional allocation, then the allocation must be proportional

\end{itemize}

\begin{proposition}
	The union property negates the proportional property.
\end{proposition}


\begin{proposition}
	The proportional property negates the union property.
\end{proposition}

\begin{definition}
min-dif allocation rule $f$.
Given valuations $v=(v_1,\ldots,v_n)$ entitlements $b=(b_1,\ldots,b_n)$, find the minimal $c$ such that there exists a partition such that each $i$ gets at least $\frac{b_i-c}{\sum_j b_j}v_i(M)$, and the valid allocation is the  allocation corresponding to this $c$.	
\end{definition}

\begin{proposition}
	The min-dif allocation rule satisfies properties: monotonicity, scaling, anonymity, proportional
\end{proposition}



*** Add description of the algorithm ***

*** add example of non Pareto output of the algorithm ***


\subsection{Research questions}



\begin{question}
For additive (submodular/subadditive) valuation functions, find upper and lower bounds on the possible ratios between the values of different types of shares.
\end{question}

The main positive result is Theorem~\ref{thm:half}.  A partial converse to it is Proposition~\ref{pro:notTruncated}.

\begin{question}
For additive valuations, can the approximation ratio against truncated proportional shares be improved to $\frac{n}{2n-1}$.
\end{question}

Obviously, better approximation ratios against other types of shares, as well as with more general valuation classes, are also desired. It may be useful to become familiar with algorithmic ideas that appear in related work.




\subsection{Related work}


Pessimistic shares (under a different name) were introduced in~\cite{BNT17}, where Proposition~\ref{pro:CE} was proved w.r.t. pessimistic shares.

In general, the notions of shares that are proposed in our work bear similarities with notions used in other contexts~\cite{Moulin90, FT14}

Our setting is similar to a line of literature that goes under the name of {\em combinatorial auctions}. Much of this literature is concerned with maximizing welfare. The configuration LP, used in this literature, is feasible when agents claim only their balanced share. Oblivious randomized rounding techniques imply that in expectation (though not deterministically), every agent can get a $\rho$ fraction of his balanced share, with $\rho = \frac{1}{2}$ for subadditive valuations~\cite{Feige09}, $\rho = 1 - \frac{1}{e}$ for XOS~\cite{Feige09}, and some $\rho < 1 - \frac{1}{e}$ for submodular~\cite{FV10}. For additive valuations one of course can ensure the balanced share in expectation by allocating each item independently at random (with probabilities equal to the entitlements). For gross substitutes valuations, even though the configuration LP is tight, rounding of it is not oblivious~\cite{FMT16}, and hence it by itself does not imply that every agent can get his fair share in expectation.

A fairness objective for combinatorial auctions is the max-min objective. However, even in the case of additive valuations, the currently known rounding techniques give very poor values, and hence do not imply anything useful in our context. The integrality gap known for the configuration LP (with max-min objective) is $\frac{1}{2}$, but this does not necessarily carry over the the balanced share (because the max-min value can be larger than the balanced share).


The work~\cite{BDO18} introduces an approximate notion of an equilibrium, but there agents are quasilinear (in our CE setting agents have no value for leftover budget). Hence the approximation results there do not seem to imply any approximation results in our setting.


A different fairness notion for the case of unequal entitlements, weighted maxmin share (WMMS), was proposed in~\cite{Farhadi+2019}. Agent $i$ partitions the items into bundles, maximizing the minimum ratio of value to entitlement, assuming that other agents keep their entitlements but have the same valuation function as $i$. This ratio times his entitlement is his WMMS value. It was shown there that for additive valuations, the best approximation factor for WMMS is $\frac{1}{n}$, and when no item is valued by an agent more than his WMMS share, one can obtain a $\frac{1}{2}$ approximation ratio. We observe that in a competitive equilibrium from unequal budgets, an agent may get less than his WMMS value. Example: two agents with entitlements $\frac{1}{4}$ and $\frac{3}{4}$, and two items with a factor larger than~3 in their values. In every CE the more entitled player takes both items, but the less entitled player has WMMS value that should give him one item.




\section{need to go over}

\begin{proposition}
\label{pro:balancedVersusSequential}
If the valuation function $v_i$ is additive, then the balanced share is at least as large as the sequential share.
\end{proposition}


\begin{proof}
Consider a partition into bundles for the sequential share, and let $\frac{p}{q} \le b_i$ be the maximal ratio over all prefixes of the adversarial order between the number of bundles taken by the agent in the prefix and the prefix length. If needed, add empty bundles to the suffix of the order so that the number of bundles $k$ is divisible by $q$, and add to the agent additional bundles so that his total number of bundles is $\frac{p}{q}k$, not taking more than a fraction of $\frac{p}{q}$ bundles from any prefix.

Make $p$ consecutive copies of each bundle, resulting in $pk$ ordered bundles. For the balanced share, take the following $q$ collections of bundles, where the $i$th collection of bundles contains all these bundles at location $i$ modulo $q$ (where bundles are numbered from~0 until $pk$). Each of them is at least as good as the sequential share.
\end{proof}

For $\alpha \ge 1$, the notion of $\alpha$-endowed equilibrium was introduced in~\cite{BDO18}. Viewing the entitlements of agents as budgets, an $\alpha$-endowed equilibrium involves an allocation of bundles to agents and prices to items with the following properties: every agent can afford his own bundle (given his budget and the prices), and the value of his bundle is at least an $\frac{1}{\alpha}$-fraction of the value of the best bundle that the agent can afford (not true, because agents are quasilinear and care about the payments).

\begin{proposition}
In every $\alpha$-endowed equilibrium CE, every agent gets at least at $\frac{1}{\alpha}$ fraction of his share  (for all types of shares listed above).
\end{proposition}

\begin{proof}
Similar to the proof of Proposition~\ref{pro:CE}.
\end{proof}

As 2-endowed equilibria exist for submodular valuations~\cite{BDO18}, we obtain the following corollary.

\begin{corollary}
If agents have submodular valuations then there is an allocation that gives every agent a bundle of value at least half of his balanced share.
\end{corollary}


\begin{question}
Can the ratio of $\frac{1}{2}$ be improved in the above corollary? Does it extend to XOS and subadditive valuations?
\end{question}

Proposition~\ref{pro:noBalancedShare} suggests that for general valuation functions, it may be useful to consider a notion of approximate fairness that approximates the entitlement, rather than the value of the share. Likewise, it suggests that rather than considering generic budgets, it might be more natural to consider approximation ratios for the entitlement.

\begin{proof}
For even integer $k > 0$, consider an instance with $m = 3k$ items partitioned into $k$ triples. There are $n=\frac{3k}{2}-1$ agents, and the valuation function $v$ of all agents is the same. Every single item has value~1, every set of two items from the same triple has value~2, every set of two items from different triples has value $\frac{3}{2}$, and every set of three or more items has value~2. It is not difficult to check that this valuation function is submodular.

For $k=8$ there are $11$ agents, each with $b = \frac{1}{11}$. Even after perturbation we have $b > \frac{2}{24}$. Create $q=24$ bundles, where every pair of items from the same triple forms a bundle. Every item appears in exactly $p=2$ bundles, and every bundle has value~2. Hence the balanced share of every agent is at least~2. However, in every allocation, at least nine of the agents do not get more than two items each, and at least one of these nine agents cannot get both items from the same triple. Hence there must be a agent that gets value at most $\frac{3}{2}$.
\end{proof}


There is an issue left open in understanding the relations between different types of shares.

\begin{question}
Does Proposition~\ref{pro:balancedVersusSequential} hold when the valuation function is not additive?
\end{question}


Given Propositions~{pro:noBalancedShare1} and~\ref{pro:entitlementNo}, there are only limited classes of valuations for which there remains hope of guaranteeing each agent his share.

\begin{question}
\label{q:GS}
Is there an allocation giving each agent his pessimistic share if valuation functions are additive? If valuations belong to some subclass of submodular (beyond unit demand which is handled in Proposition~\ref{pro:unitDemand})? What about sequential share?
\end{question}


For other classes, one may consider approximations. Two types of approximations come to mind: one is to approximate the value of the share, and one is to approximate the entitlement (Proposition~\ref{pro:entitlementNo} shows that this last notion of approximation has limited applicability).

\begin{question}
Is there an allocation that gives each agent a $\rho$-fraction of the value of his share (balanced, sequential or pessimistic) for interesting classes of valuation functions (such as submodular/XOS/subadditive)?
\end{question}

\begin{theorem}
\label{thm:half}
With arbitrary entitlements and additive valuations, there is an allocation giving each agent at least half his balanced share.
\end{theorem}

\begin{proof}
For each agent, truncate values of items so that no item is worth more than his balanced share. The value of the balanced share does not change. With respect to the new valuations, we show that each agent can get at least half his proportional share, and hence also at least half of balanced share.

Sort the agents in order of decreasing entitlements, and scan agents one by one. For each agent, if there is an item of value (for him) at least half his proportional share, give the agent the item and remove the agent. If there is no such item, break the agent into two subagents, each with half the entitlement, and insert them in the appropriate place in the sorted order. (The bundle that the agent receives will be the union of the bundles received by the two subagents, recursively.)

In every step $t$, for every agent (or subagent) $i$, either he gets half his proportional share (and leaves), or his proportional share does not change (if an agent was split at that step), or his proportional share does not decrease (when another agent $j$ takes an item and leaves). To see that the last statement holds, let $p_i$ and $p_j$ be the proportions to which $i$ and $j$ where entitled to at the beginning of step $t$. Observe that $p_j \ge p_i$. Moreover, if $V_i$ denotes the value for $i$ of all remaining items, then the item taken by $j$ could not have value greater than $p_i V_i$. Indeed, no item has such high value. This can be shown by induction on the number of rounds. Initially, this holds because of truncation. When an agent is split this holds because before the split no item was worth to the agent more than half the proportional share. When a different agent takes an item, this holds because the values of other items do not change, and the relative proportion of the agent does not decrease.
\end{proof} 

\begin{enumerate}

\item If there is an item such that winning it completes the value to at least $\frac{3}{4}$, bid all your budget.

\item If there is an item of value at least $\frac{5}{8}$, bid $\frac{5}{8}-\epsilon$.

\item If there is an item of value larger than $\frac{1}{2}$, bid $\frac{1}{2}+\epsilon$ (but no more than the value of the item).

\item Bid the value of the highest valued item.

\end{enumerate}

Steps~1 and~4 above are natural. Steps~2 and~3 are added so as to give the bidder a buffer from $\alpha$ after winning his first item. Removing step~2 does not give $\frac{3}{4}$ if there are $k-1$ bundles, each with three items of value $\frac{3}{4}^-$, $\frac{3}{16}^-$ and $\frac{1}{16}^+$, and one bundle with 10 items of value $\frac{1}{10}$ (the choice of 10 is not optimized). The adversary can start by winning the heavy items, then bid $\frac{1}{4}^-$ on the medium items, and even if he wins all these items he needs to give up only 10 of the remaining items of value $\frac{1}{16}^+$. The above strategy also fails if each bundle has an item of value $\frac{5}{8}$, and many bundles have in addition three items of value $\frac{1}{8}^-$. The adversary lets us win the first item, then each adversarial agent wins a heavy item, and then some adversarial agents win four medium items.


==> sec-additive.tex <==

\section{A Truthful Mechanism for Dichotomous Additive Valuations}
\label{sec:additive}
In this section we  design a deterministic allocation mechanism that is truthful when players dichotomous additive valuations.
The allocation of the mechanism is welfare maximizing and gives each truthful player at least his max-min share.

For the case of dichotomous additive valuations, the valuation can be concisely represented by the set of items the player demands. 
Every player is asked to report his set of demanded items, and he provides a report $R_v \subset M$. If $R_v = D_v$ we say that the player is \emph{truthful}. The allocation \emph{mechanism is truthful} if being truthful is a weakly-dominant strategy for every player.

For dichotomous additive valuations, given the reports of players, an allocation $A$ is {\em reasonable} if every player $v$ gets only items from his own reported set, that is, $A_v \subseteq R_v$.

% MB old:
%if the following two conditions hold:

%\begin{enumerate}

%	\item All reported items are allocated, and no other item is allocated. $\bigcup R_v = \bigcup A_v$.

%	\item Every player gets only items from his own reported set. $A_v \subseteq R_v$.

% \end{enumerate}

The {\em profile} of an allocation $A$ is the vector $(|A_1|, \ldots, |A_n|)$ specifying how many items each player gets. Two allocations that have the same profile are said to be {\em equivalent}. If a player is truthful then the values that he derives from two equivalent allocations are the same.


% MB: removing this:
% OLD: (All our results extend to valuation functions of the form $f(|A_v \cap D_v|)$ where $f$ is an arbitrary nonnegative monotone nondecreasing function.)
The max-min share of player $v$ is $\lfloor \frac{|D_v|}{n} \rfloor$. Note that if $m < n$ then the max-min share of every player is~0 \mbcomment{so? We still want to maximize welfare (allocate all items) while the mechanism being truthful. Can we remove this assumption? Are we ever using it?}, and hence we may assume that $m \ge n$.

\mbedit{An allocation is \emph{envy free up to one good, abbreviated by EF1,} if no player $i$ prefers the bundle of another player $j$ after removing some item from the bundle of $j$.}


We now present the {\em balanced mechanism}, that maps reports of players to allocations. Informally, it fixes some arbitrary priority order among the players (for simplicity, player~1 has highest priority, player $n$ has lowest priority). Thereafter, given the reports of players, it selects a welfare maximizing reasonable allocation whose profile is as balanced as possible, trying to equalize the amount of items that each player gets, subject to the allocation being welfare maximizing and reasonable, and breaking ties in favor of players of higher priority.

In more details, the balanced mechanism is defined as follows. Identifying the set of players $V$ with the set $[n]$, for an allocation $A$, we define its potential as:

$$\pi(A) = \sum_{i \in V} (n|A_i| + i)^2$$

Observe that the potential is a function only of the profile of the allocation, and equivalent allocations have the same potential. Given the reports of the players, the balanced mechanism selects an arbitrary allocation among those welfare maximizing reasonable allocations that minimize the potential.
\tecomment{maybe add the priorities as inputs to the mechanism?}
\begin{theorem}
\label{thm:truthful01}
The following properties hold for the balanced mechanism.

\begin{enumerate}
\item \label{item:truthful} For players with dichotomous additive valuations, being truthful is a dominant strategy.

\item \label{item:welfare} When players are truthful the allocation is welfare maximizing and reasonable.
	
\item \label{item:fair}  Every truthful player gets at least his max-min share \mbedit{and the allocation is EF1 (envy free up to one good)}.

\item \label{item:poly}  The output of the mechanism can be computed in polynomial time.

\item \label{item:equivalent}  Every two allocations that are legal outputs of the mechanism are equivalent (have the same profile).

\end{enumerate}

\end{theorem}

We derive the proof of the theorem from several claims we prove next.


The following proposition restates and proves item~\ref{item:fair} of Theorem~\ref{thm:truthful01}.

\begin{proposition}
\label{pro:maxmin01}
	In the balanced mechanism, every truthful player $v$ gets at least his max-min share \mbedit{and the allocation is EF1 (envy free up to one good)}.
\end{proposition}

\begin{proof}
Let $A$ be the allocation output by the balanced mechanism. For a truthful player $v$, his reported set $R_v$ is his demand set $D_v$. As $A$ is welfare maximizing, all of $D_v$ is allocated, and as it is reasonable $A_v \subseteq D_v$. We claim that $v$ receives at least $t = \lfloor \frac{|D_v|}{n} \rfloor$ items from $D_v$ (which is his max-min share). Assume for the sake of contradiction otherwise. Then as all of $D_v$ is allocated, some other player, say $u$, must receive at least $t+1$ items from $D_v$, whereas $v$ receives at most $t-1$ items altogether. This contradicts the requirement that $A$ minimizes the potential, as we may transfer some item of $D_v$ from $u$ to $v$, and by this get an allocation of lower potential.

 \mbedit{Finally, observe that the allocation is EF1. If player $v$ envies player $u$ even after an item is  removed from the set that $u$ got, then $u$ got at least two items more than $v$, and moving an item that $v$ desires from $u$ to $v$ is feasible and decreases the potential, in contradiction to the assumption that the allocation has minimal potential.}
\end{proof}


The following lemma restates and proves item~\ref{item:poly} of Theorem~\ref{thm:truthful01}.

\begin{lemma}
	\label{lem:BalancedAlgorithm}
	There is a polynomial time algorithm (polynomial in $n$ and $m$) that given the requested sets of the players, computes a welfare maximizing reasonable allocation of smallest potential.
\end{lemma}

\begin{proof}
	We shall present an iterative algorithm that converges in a polynomial number of steps to a welfare maximizing reasonable allocation of smallest potential.
	
	Start by allocating each requested item to an arbitrary player that requests it. Then, in every iteration do the following.
	
	Given the allocation $A$ in the beginning of the iteration, construct a directed graph in which the agents are the vertices, and there is a directed edge from agent $u$ to agent $v$ if agent $u$ holds some item $j$ that is in the intersection of their requested sets, $j \in R_u \cap R_v$. If a vertex $t$ is reachable in this graph from vertex $s$, then the solution can be modified into one in which $t$ gains an item and $s$ loses an item. In this case we say that $s$ can (indirectly) transfer an item to $t$. If a transfer of one of at least the following two types is possible, perform one such transfer arbitrarily, and end the iteration.
	
	\begin{enumerate}
		
		\item {\em Strong transfer}. $s$ has at least two items more than $t$.
		
		\item {\em Weak transfer}. $s$ has one item more than $t$, but lower priority than $t$.
		
	\end{enumerate}
	
	If no strong and no weak transfer is possible, the algorithm ends.
	
Observe that strong and weak transfers lower the potential. As the potential function $\pi$ receives only integer values and its maximum possible value is at most $O(n^2m^2)$, the algorithm ends in a polynomial number of steps. Each step can be implemented in polynomial time, using standard connectivity algorithms for directed graphs.

The fact that when the algorithm ends we have a welfare maximizing reasonable allocation with smallest potential follows from Lemma~\ref{lem:paths} \mbcomment{this is a forward pointer, consider changing the order}. (A canonical path in the graph of Lemma~\ref{lem:paths} translates to a path in our graph that decreases potential.)
\end{proof}


We now develop some background that will allow us to establish that the balanced mechanism is truthful.

Let $A^1$ and $A^2$ be two reasonable allocations, where $A^i(e)$ denotes the agent that receives item $e$ under allocation $A^i$. Given $A^1$ and $A^2$, consider a directed multi-graph $G_{A^1,A^2}(V,E)$ (that we shall refer to as $G$ for brevity) with edge labels $\ell : E \rightarrow M$. (Note: this graph is different from the one appearing in the proof of Lemma~\ref{lem:BalancedAlgorithm}.) The vertices of $G$ are the agents $V$. For every item $e \in M$, if $A^1(e) \not= A^2(e)$ then we introduce a directed edge $(A^1(e), A^2(e))$ and label it by $e$. (If $A^1(e) = A^2(e)$ then  $(A^1(e), A^2(e))$ would be a self loop, which we omit.) For an agent $v$, let $s_v$ denote the difference between $v$'s out-degree and in-degree in $G$.  Then $s_v = |\{e | A^1(e) = v\}| -  |\{e | A^2(e) = v\}|$. We refer to $v$ as a {\em source} if $s_v > 0$ and as a {\em sink} if $s_v < 0$.
Let $d = \sum_{v | s_v > 0} s_v$ and observe that  $d = \sum_{v | s_v < 0} |s_v|$ \mbcomment{I think writing this as $d = -\sum_{v | s_v < 0} s_v$ is clearer }. By arguments similar to those for Eulerian cycles, it follows that the edges of $G$ decompose into $d$ edge disjoint source to sink simple paths, and possibly some additional cycles. There may be several such decompositions, and we fix one of them arbitrarily. We refer to each path in this decomposition as a {\em canonical transfer path}. Implementing the transfers along the edges of a path, the potential changes because the source of the path loses one item and the sink gains one item (and the potential function is such that this cannot leave the potential unchanged).  Starting from $A^1$ and implementing the transfers of items along the edges of every canonical transfer path, we reach an allocation that has exactly the same potential as $A^2$. (Implementing the transfers along a cycle does not change the potential of an allocation.)

Given $A^1$, $A^2$, $G$ and the set of canonical transfer paths ${\cal{P}} = \{P_1, \ldots, P_d\}$ as above, consider the set function $g : {\cal{P}} \rightarrow R$, where for a set $S \subset {\cal{P}}$ we define $g(S) = \pi(A^S) - \pi(A^1)$ \mbcomment{need to decide if this is reversed and adjust the following proposition and lemma accordingly }, where $\pi$ is the potential function and $A^S$ is the allocation after all transfers along the paths of $S$ are implemented.

\begin{proposition}
The function $g$ is supermodular.
\end{proposition}

\begin{proof}
Let $S \subset T \subset {\cal{P}}$ and consider a path $P_i \not\in T$. We need to show that the marginal values satisfy $g(P_i | T) \ge g(P_i | S)$. This follows because the canonical paths in $T \setminus S$ can only decrease the number of items in the source of $P_i$, and only increase the number of items in the sink of $P_i$. Hence the marginal decrease in potential due to the source only decreases, and the marginal increase due to the sink only increases.
\end{proof}

The following lemma proves item~\ref{item:equivalent} of Theorem~\ref{thm:truthful01}, among other things.

\begin{lemma}
\label{lem:paths}
There is a unique profile for welfare maximizing reasonable allocations that minimizes the potential. Moreover, given any welfare maximizing reasonable allocation $A^*$ with this minimum potential, any other allocation $A^1$ with a different profile, every canonical path in the associated directed graph $G_{A^1,A^*}$ strictly decreases the potential.
\end{lemma}

\begin{proof}
Let $A^*$ be a welfare maximizing reasonable  allocation whose profile has smallest potential (we do not assume here this profile is unique -- this will follow from the proof), and let $A^1$ be some welfare maximizing reasonable  allocation with a different profile. Let ${\cal{P}}$ be the set of canonical paths in $G_{A^1,A^*}$. As $A^*$ has smallest potential, $g({\cal{P}}) \le 0$. Observe that no single path $P_i$ can have  $g(P_i) = 0$ (by nature of the potential function $\pi$). Suppose for the sake of contradiction that there is a canonical path $P_i$ with $g(P_i) > 0$. Then as long as there is a canonical path with negative $g$ value, implement its transfers. By supermodularity, we will eventually remain only with canonical paths with positive $g$ value. But then, implementing them increases the potential, showing that $A^*$ could not have minimum potential.

The above argument (using the fact that no single path $P_i$ can have  $g(P_i) = 0$)  also implies that $A^1$ cannot have the same potential as $A^*$, showing the uniqueness of  the potential minimizing profile.
\end{proof}

We say that an allocation rule is {\em monotone} if whenever a player increases his requested set by one item, the size of the set allocated to him does not decrease. We say that an allocation rule is {\em Lipschitz} if whenever a player increases his requested set by one item, the size of the set allocated to him increases by at most one item. We say that an allocation rule is {\em faithful} if whenever a player $v$ replaces his requested set $R_v$ by his allocated set $A_v$, then under this new request (and having the remaining request sets unchanged) the allocated set \mbedit{to player $v$ does not change and remains $A_v$}.

\begin{lemma}
\label{lem:true01a}
The balanced mechanism is monotone, Lipschitz and faithful.
\end{lemma}

\begin{proof}
{\em Faithful.} Let $A$ be the allocation when $v$ reports $R_v$  (and getting $A_v$), and let $B$ be the allocation when $v$ reports $A_v$ (and getting $B_v$).
As $A$ is feasible in the second setting and $B$ is feasible in the first setting, Lemma~\ref{lem:paths} implies that $A$ and $B$ have the same profile. As such, $v$ receives $|A_v|$ items in $B$, and this can only happen if $B_v = A_v$.

We now turn to Lipschitz and monotonicity. Fixing the reports of all agents, let $A$ denote a minimum potential allocation. Now let agent $v$ add item $e$ to his report, and let $B$ denote the resulting  minimum potential allocation. If $e \not\in B_v$ then Lemma~\ref{lem:paths} implies that $A$ and $B$ have the same profile, because $B$ was also avaliable in the original setting and $A$ is avaliable in the final setting. Hence $|B_v| = |A_v|$, establishing both Lipschitz and monotonicity in this case.

It remains to handle the case that $e \in B_v$.

{\em Lipschitz.}
Suppose for the sake of contradiction that $|B_v| > |A_v| + 1$. Consider an allocation $A^1$ that is the same as $A$, except that for item $e$ we fix $A^1(e) = v$. Consider the canonical paths in $G_{A^1,B}$. By Lemma~\ref{lem:paths}, each of them decreases the potential. Also, at least one of them, say $P_1$, must have $v$ as a sink.  The paths do not involve $e$ (as $A^1(e) = B(e) = v$), and hence can also be implemented between $A$ and $B$ instead of between $A^1$ and $B$.  Implementing $P_1$ in $A$ decreases the potential, because it does so in $A^1$, and the sink of $P_1$ has more items in $A^1$ than it has in $A$, whereas the source of $P_1$ cannot have more items in $A^1$ than in $A$. This contradicts the assumption that $A$ had smallest potential among all reasonable allocations.


{\em Monotone.}
Suppose for the sake of contradiction that $|B_v| < |A_v|$. Consider an allocation $A^1$ that is the same as $A$, except that for item $e$ we fix $A^1(e) = v$. Consider the canonical paths in $G_{A^1,B}$. By Lemma~\ref{lem:paths}, each of them decreases the potential. Also, at least $|A_v| + 1 - |B_v| = t \ge 2$ of them, say $P_1, \ldots, P_t$, must have $v$ as a source.  If it happens that any of these paths have as a sink the vertex $A(e)$, then without loss of generality we assume that $P_1$ is such a path.
The paths do not involve $e$ (as $A^1(e) = B(e) = v$), and hence can also be implemented between $A$ and $B$ instead of between $A^1$ and $B$.

We claim than implementing $P_t$ in $A$ decreases the potential (contradicting the assumption that $A$ had smallest potential among all reasonable allocations). This follows from the following two observations. One is that first implementing $P_1, \ldots, P_{t-1}$ in $A_1$ to obtain $A'$ and then implementing $P_t$ in $A'$ decreases the potential of $A'$ (this follows from $B$ having the smallest potential). The other is that the source of $P_t$ has the same number of items in $A$ and in $A'$, whereas the sink $u$ of $P_t$ cannot have less items in $A'$ than in $A$. (If $u = A(e)$ then in $A^1$ it has one less item than in $A$. However, by the rule for choosing $P_1$, it gains an item by the time $A'$ is reached.)
\end{proof}

\begin{lemma}
\label{lem:true01b}
If a deterministic  allocation mechanism only outputs reasonable allocations and is monotone, Lipschitz and faithful, then for every player with a 0/1 additive valuation function, being truthful is a dominant strategy.
\end{lemma}

\begin{proof}
Fix the report of all players. Let $R_v$ be an arbitrary report of player $v$, let $A$ be the resulting allocation, and let $A_v$ be the set of items allocated to $v$.  Let $B$ be the allocation in case that the report of $v$ is his demand set $D_v$, and let $B_v$ be the set of items allocated to $v$ in this case. We need to show that $|B_v \cap D_v| \ge |A_v \cap D_v|$.

Note that $A_v \subset R_v$ because the allocation is reasonable. First change $R_v$ to $A_v$. By faithfulness of the mechanism, the allocation to $v$ remains $A_v$. Now change the report $A_v$ to be $A_v \cap D_v$. By the Lipschitz property combined with reasonableness it must be that the allocation to $v$ becomes $A_v \cap D_v$. Now change the report to $D_v$. By monotonicity, the number of items allocated to $v$ does not decrease, and as all of them are in $D_v$, his value does not decrease.
\end{proof}

\mbedit{We remark that the three properties (monotone, Lipschitz and faithful) are each necessary for truthfulness. Monotonicity  is clearly needed. If a  mechanism is not faithful, then when player $v$ really wants $A_v$ he can increase his value by declaring $R_v$. Finally, the allocation must be Lipschitz as   ... FINISH!  }

We now derive the proof of  Theorem~\ref{thm:truthful01} from the above claims.

\begin{proof}
Truthfulness (item~\ref{item:truthful}) follows by combining Lemmas~\ref{lem:true01a} and~\ref{lem:true01b}.
When players are truthful, the fact that the allocation is welfare maximizing and reasonable (item \ref{item:welfare}) is immediate from the definition of the mechanism.
Fairness properties (item~\ref{item:fair}) is proven in Proposition~\ref{pro:maxmin01}.
Polynomial-time computation (item~\ref{item:poly}) is proven in Lemma~\ref{lem:BalancedAlgorithm}.
Finally, equivalence of allocations (item~\ref{item:equivalent}) is proven as part of Lemma~\ref{lem:paths}.
\end{proof}

\mbcomment{Should we talk about the stronger fairness property the mechanism has: if a player has an item that another player wants, then the first player as at most one item more than the second player. Is this actually a lex-max solutions? BTW - What are the relations between lex-max and max-min and EF1? Does lex-max always imply the others?}

The next example shows that there is no truthful welfare maximizing mechanism with dichotomous additive valuations when adding (arbitrary, not Matroid) downward-closed constraints.
\begin{example}% [no truthful welfare maximizing with 0/1 additive valuations under downward-closed constraints]
	\label{ex_general_constraints}
	A market with two agents and five items, feasible sets $F=\{\{1\},\{2,3,4,5\}\}$ (and all of their subsets), and allocations that maximize welfare.
	% and are reasonable.
	If both agents want items $\{2,3,4,5\}$ then w.l.o.g., agent~1 gets at least two items. If agent~1 wants in addition also item 1, the maximum welfare allocation changes, gives item~1 to agent~1, and the remaining four items to agent~2. Hence agent~1 gets higher value by not reporting item~1.
\end{example}

\mbc{I have copied this example to the appendix so we will be able to remove this section. }

==> sec-intro.tex <==
\subsection{OLD Introduction}

Our goal in this work is to design allocation mechanisms\footnote{\mbedit{We are considering only settings without money, so a mechanism can only define the allocation rule, but cannot define any payment rule as there are no payments.}} that are easy to implement in practice, and also enjoy desirable theoretical properties, related to their economic efficiency, to fairness of the allocation, and to incentive compatibility. Achieving these theoretical guarantees simultaneously is impossible if agents may have general valuation functions over the set of items to be allocated. Hence we consider a setting in which agents have {\em additive dichotomous} valuations (to be defined shortly), and some extensions of this basic setting. As a motivating example, suppose that there is an arts museum that is interested in employing arts students as guides in the museum. There are different shifts for this employment (for simplicity, suppose that there is one shift per day, and the different shifts correspond to different days), at most one student can be employed per shift, and students receives payment for their work (same amount for every shift). There is a pool of arts students who are interested in this form of employment, and are all roughly equally qualified for the job (they all passed some initial screening). Some of the shifts might not be desirable for a given student (e.g., some students do not want to work on weekends, some do not want to work on days in which they have exams, some do not want to work on days when there favorite basketball team is playing), but the remaining shifts are equally desirable for the student. The goal of the museum is to fill up as many shifts as possible (one student per shift), and the goal of each student is to receive as many shifts as possible (thus maximizing income), among those shifts desirable for the student. We assume that allocation of shifts to students is done in a batch fashion, say, one a month. In the beginning of the month each student reports which shifts are desirable, and based on the reports, the museum generates a schedule for the whole month.

The task of generating a schedule for a month is formalized in this work as follows. There is a set $V$ of $n \ge 2$ players, also referred to as agents. In our example, this set corresponds to the pool of students who are interested in employment as museum guides. There is a set $M$ of $m$ items, which in our example corresponds to the different shifts available in the upcoming month. Each player $v \in V$  has a \emph{demand set} $D_v \subseteq M$, which in our example corresponds to the shifts desirable by the particular student. This demand set induces {\em additive dichotomous valuation function} for agent $v$: every item $v \in D_v$ has value~1, every item $v \not\in D_v$ has value~0, and the value of a set of items is the sum of values of items in the set. (In our example, it is reasonable to model undesirable items as having value~0 for the agent rather than negative value \tecomment{not the other way?}. We do not assume that all shifts must filled -- it is okay if on some days there are no guided tours. A student who receives a shift may ``return" it to the museum, e.g., by claiming not to feal well on that day. The museum may then either leave this shift unallocated, or possibly assign it to a different student who is on a waiting list for this shift.)
An \emph{allocation} $(A_i,A_2,\ldots, A_n)$ % $A : M \rightarrow V$ 
assigns items to players, possibly leaving some items unallocated. 
We denote by $A_v$ the set of items allocated to player $v$ under allocation $A$. The \emph{value} of allocation $A$ for player $v$ is $|A_v \cap D_v|$.

Given the demand sets of the players, which allocation should we choose? We employ two classes of criteria for this choice. One class refers to economic efficiency, and the other refers to fairness. We discuss both this classes below.


{\bf Economic efficiency.} In our setting of additive dichotomous valuations, several common notions for economic efficiency coincide. We say that an allocation $A$ is {\em Pareto optimal} if no allocation $A'$ gives each agent at least as high value as in $A$, and strictly improves the value for at least one agent. We say that an allocation is \emph{welfare maximizing} if there is no other allocation of larger welfare, where we define the \emph{welfare} of an allocation $A$ as $\sum_v |A_v \cap D_v|$ (this definition assumes that valuation functions of different agents are measured in the same scale). We say that an allocation $A$ is {\em reasonable} if every item that is in some demand set is allocated to an agent that demands it. It is not difficult to see that when agents have additive dichotomous valuations, an allocation is Pareto optimal iff it maximizes welfare iff it is reasonable. Our economic efficiency requirement is that the allocation is reasonable (and hence also Pareto optimal and welfare maximizing).
%{\em reasonable for the agents} -- every agent receives only items that are in his/her demand set.
%Our economic efficiency requirement is that the chosen allocation is one that maximizes welfare. Often it is the case that the notion of welfare is based on the assumption that all agents use the same scale in specifying their valuation functions. The common scale is typically units of money. In our setting maximizing welfare has an additional interpretation that need not make the common scale assumption. The welfare corresponds to the number of items that are allocated, assuming that an agent ``returns" those items allocated to him/her that are not from his/her demand set.
%Maximizing the number of allocated items may be a goal by itself. In the Museum example,  having guided tours offers its visitors a more rewarding experience, so just having tours on as many days of possible is a legitimate welfare goal.

%Note that for 0/1 additive valuations, any allocation that leaves no demanded item unallocated is welfare maximizing.}

{\bf Fairness.} We are interested in ex-post notions of fairness (though some ex-ante notions of fairness will be touched upon in later parts of this manuscript.) That is, the chosen allocation (rather than just the process of choosing it) needs to satisfy some fairness condition. The simplest of these notions is {\em max-min fairness}.
The {\em max-min share} of a player $v$ is the maximum value that $v$ can derive if $v$ partitions the set of all items into $n$ bundles, and $v$ gets the bundle of least value (according to $v$'s valuation function) among these bundles. In the context of additive dichotomous valuations, the max-min share of player $v$ is $\left\lfloor \frac{|D_v|}{n} \right\rfloor$, and an allocation $A$ is max-min fair if for every agent $v$ we have that $|A_v\cap D_v| \ge \left\lfloor \frac{|D_v|}{n} \right\rfloor$. Another fairness notion is that of {\em envy-free}, which means that no player $i$ prefers the bundle of another player $j$. Envy free solutions are also max-min fair, though they often do not exists (e.g., when there are two players and only one item). Hence envy freeness is typically relaxed to
{\em envy-free up to one good} (EF1) \tecomment{EFX?}, which means that no player $i$ prefers the bundle of another player $j$ after removing some item from the bundle of $j$. An allocation may be max-min fair but not EF1, and vice versa. For additive dichotomous allocations EF1 translates to $|A_i \cap D_i| \ge |A_j \cap D_i| - 1$ for every two agents $i$ and $j$, and this (together with the assumption that every demanded item is allocated) does imply max-min fairness for these valuations.  An agent interested in max-min fairness cares only about what bundle he himself receives, and how many other agents share the remaining items. An agent interested in EF1 cares also about how the remaining items are allocated to the other agents. In our work we shall consider both max-min fairness and EF1. We remark that additional notions that are often associated with fairness will come up at a later point in this manuscript.


So far we assumed that the demand sets of agents are known. In our work we do not make such an assumption, and instead assume that each agent $v$ is asked to supply to the allocation mechanism his demand set $D_v$, and in reply supplies a report $R_v$. We say that a player is {\em truthful} if $R_v = D_v$. We say that an allocation mechanism is {\em incentive compatible} (or {\em truthful}) if being truthful is a weakly dominant strategy for every agent.


Go over the following points:
\begin{itemize}
	\item No truthful mechanism for 2 agents that gives each his maxmin share (\cite{Ghodsi+2018}).
	\item For 3 agents, it is not possible to give all 3 agents their maxmin share concurrently (\cite{KPW18}).
	\item We show that for 2 agents, it is not possible to give both agents their maxmin share with a deterministic truthful mechanism (Proposition \ref{prop:level}). \mbc{i think we will remove this} % \mbcomment{For this to be interesting we need to prove the impossibility holds for leveled valuations}
	\item We want to find an interesting domain in which it is possible to give every agent his maxmin share (and be EF1) and do this with a deterministic truthful mechanism (discuss the problem with randomization and the desire for ex-post fairness - maybe using risk aversion).
	\item We present such results for 0/1 additive valuations (Theorem \ref{thm:truthful01}).
	\item This result cannot be extended if we add downward closed constraints (Example \ref{ex_general_constraints})
	\item This result cannot be extended even to \emph{almost} 0/1 additive valuations (for three agents as we cannot give all their maxmin share \cite{KPW18}, and for 2 agents as Proposition \ref{prop:level} holds for almost 0/1 additive valuations). So we aim for giving each agent ''almost his maxmin share''. Running the deterministic mechanism of Theorem \ref{thm:truthful01} is no longer truthful.
	\item Yet, we can do it with a randomized truthful mechanism (Theorem \ref{thm:truthfulAmost01}).  Main point - giving each agent ''almost his maxmin share''  not only in expectation, but for every realization.
	\item Not possible to combine leveled with MRF - for leveled MRF there is no truthful randomized mechanism that allocates the maximal number of items ex-post.
	\item Talk about motivation for 0/1 additive valuation with fairness: allocation of shifts (we will need to assume that every shift is desirable by some agent). Extend to multiple positions in a shift (each item has multiple copies).  Can we use course allocation to students instead of shifts? Another possible domain: allocation of kidneys to hospitals. They want to maximize the number of kidneys they get. There might be a constraint that every patients needs at most one kidney. Problems: who has the kidneys in the first place? why share equally between hospitals?
	
\end{itemize}
 

